Deep learning-based surrogate model for 3-D patient-specific computational fluid dynamics

Optimization and uncertainty quantification have been playing an increasingly important role in computational hemodynamics. However, existing methods based on principled modeling and classic numerical techniques have faced significant challenges, particularly when it comes to complex 3D patient-specific shapes in the real world. First, it is notoriously challenging to parameterize the input space of arbitrarily complex 3-D geometries. Second, the process often involves massive forward simulations, which are extremely computationally demanding or even infeasible. We propose a novel deep learning surrogate modeling solution to address these challenges and enable rapid hemodynamic predictions. Specifically, a statistical generative model for 3-D patient-specific shapes is developed based on a small set of baseline patient-specific geometries. An unsupervised shape correspondence solution is used to enable geometric morphing and scalable shape synthesis statistically. Moreover, a simulation routine is developed for automatic data generation by automatic meshing, boundary setting, simulation, and post-processing. An efficient supervised learning solution is proposed to map the geometric inputs to the hemodynamics predictions in latent spaces. Numerical studies on aortic flows are conducted to demonstrate the effectiveness and merit of the proposed techniques.

==> discussion.tex <==
\subsection{Fast surrogate for local hemodyanmics prediction}
In this study, an ML-based surrogate model is developed for hemodynamic predictions given a aorta shape, which is trained and tested on sample sets with a variety of sizes. 

\underline{Predicting local hemodynamic information.} In contrast to traditional surrogate model (e.g., GP models) or reduced-space model (e.g., LP/1D models), the proposed ML-based surrogate model is able to rapidly predict local hemodynamic information such as blood flow pattern, surface pressure and WSS distributions over the vessel walls. As shown in Figure~\ref{fig:three sin x}, the hemodynamic fields predicted by the DNN are compared to the CFD reference as the ground truth. 
%The field outputs from the neural network are compared to the ground truth which is the CFD solution projected on the regulated meshes. The visualization of the field outputs is reported in Figure 6. 
Four samples are randomly selected for illustration and the prediction from neural networks and the ground truth from CFD are compared. Besides, absolute error contours are also plotted out by substracting the ground truth from the prediction. For pressure contours, the surrogate model yields very close surface distribution to the ground truth, yet slight differences exist at the stenosis of the descending aorta. Judging from the error contours, this discrepancy is mild on sample 1 but conspicuous on sample 3, which means the surrogate model has its limitations in capturing local details with large pressure gradients, where there are more flow vortices induced by sharp changes of surface curvatures, stenosis for instance, in the aorta geometry such as sample 3. Prediction of the wall shear stress distribution is in good agreement with the ground truth. However, the surrogate model smooths out the small fluctuations of wall shear stress from the CFD solutions.

\begin{figure}[htp!]
\centering
\includegraphics[width=0.8\linewidth]{figures/paw_clip.pdf} 
\caption{ML surrogate predictions of pressure (top) and wall shear stress (bottom) are compared with the CFD ground truth: prediction (1st and 4th row), CFD ground truth (2nd and 5th row), prediction error (3rd and 6th row)}\label{fig:pressure}
\end{figure}
\begin{figure}[htp!]
\centering
\includegraphics[width=0.8\linewidth]{figures/vam_clip.pdf} 
\caption{Cross-section velocity magnitude (top) and velocity vector filed (bottom) comparison of prediction and CFD ground truth: prediction (1st and 4th row), ground truth (2nd and 5th row), error (3rd row)}\label{fig:velocity}
\end{figure}


It appears that high-frequency components of the output are partially canceled out when interpolating among neighboring training samples based on the non-linear relations learned by the neural network. Similar to pressure, obvious inconsistency is also observed near the stenosis on the descending aorta for sample 3. The velocity contours on the cross-section and internal velocity vector field are visualized in Figure 7. As expected, the planar velocity contours show that the predicted flow velocities near the stenosis are more biased compared to the ground truth. Nonetheless, the overall flow velocity vector fields from the neural network and CFD are very consistent for all samples viewing the glyph pictures at the bottom of Figure 7.

\clearpage 

\subsection{Comparison with the bi-fidelity model}
To investigate how well the proposed model performs among other state-of-art surrogate models, a bi-fidelity surrogate model proposed by Han\cite{HanBF} is chosen for comparison. The multi-fidelity paradigm is pioneered by M.C. Kennedy\cite{KennedyMF} originally from a statistical point of view (e.g., GP-based multi-model approach) decades ago. The application of multi-fidelity models on inverse flow and uncertainty quantification (UQ) problems are developed and evolved more recently. The theoretical backbone of the adopted bi-fidelity model is based on the multi-fidelity paradigm, which leverages the accuracy of the high-fidelity CFD solutions and the efficiency of the low-fidelity solutions, largely reducing the total computation cost of conventional image-assisted CFD forward simulation models similar to the ML-based surrogate model. Yet the efficiency of the bi-fidelity model is inferior to that of the ML-based surrogate model because one still has to inevitably conduct low-fidelity CFD simulations not needed for the ML-based surrogate model. To build the bi-fidelity model, another 1000 CFD simulations are conducted on low-resolution meshes, from which the FOIs are extracted from the simulation results. The low-fidelity CFD cases are calculated on very coarse meshes and are stopped at early iterations before reaching convergence to reduce the online time. Combined with the existing high-fidelity cases, a bi-fidelity surrogate model is built and compared with our proposed model. To find out how the prediction errors change with the training size, the training set size is set to change from 300 to 900 and the testing set is a fixed group of 100 samples randomly selected from the total dataset. The comparison of performance is illustrated in Figure 8. Both surrogate models have reasonably good predictions but the surrogate model with neural network (NN) has a better performance for all conditions, hence is more recommended. Both surrogate models reach their best accuracy at $TS=900$ for all FOIs. The error of the bi-fidelity (BF) model quickly rises as the training size decreases while that of the NN model rises mildly, indicating a more robust behavior at low sample numbers. For both models, the 3-D velocity vector field is easier to fit than surface field outputs such as pressure and wall shear stress due to the fact that they are more sensitive to the local changes of the input shape cross difference patients. In general, all FOIs are well predicted with acceptable errors and the proposed ML-based surrogate model is superior to the bi-fidelity model. 

\begin{figure}[ht]
     \centering
     \begin{subfigure}{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/psen3.pdf}
         \caption{Pressure}
         \label{fig:psen}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/usen3.pdf}
         \caption{Velocity}
         \label{fig:usen}
     \end{subfigure}
\hfill
     \begin{subfigure}{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/wsen3.pdf}
         \caption{Wall shear stress}
         \label{fig:wsen}
     \end{subfigure}
        \caption{Comparison of neural network(NN) and bi-fidelity model(BF): Y axis, averaged mean square error (AMSE); X axis, trainset size (TS)}
        \label{fig:puwsen}
\end{figure}


















\begin{figure}[h]
\centering
\includegraphics[width=0.95\linewidth]{figures/pwv_clip.pdf} 
\caption{Comparison of prediction and ground truth}
\end{figure}

\subsection{Regression of geodesic characteristic}

==> headers/header-common.tex <==
% !TEX root = mfu-main.tex
% Above is for TeXShop to find the main file. Don't touch


% \usepackage[top=1in, bottom=1in, left=1in, right=1in]{geometry}
% \usepackage[top=1in, bottom=1in, left=0.35in, right=2in]{geometry}

\usepackage{graphicx}
\usepackage{amsmath}

\usepackage{natbib}
%% The amssymb package provides various useful mathematical symbols
\usepackage{amssymb}

%% The amsthm package provides extended theorem environments

\usepackage{amsthm}

%% The lineno packages adds line numbers. Start line numbering with
%% \begin{linenumbers}, end it with \end{linenumbers}. Or switch it on
%% for the whole article with \linenumbers after \end{frontmatter}.
\usepackage{lineno}
\usepackage{subfig}
\usepackage{enumerate}
\usepackage{fullpage}
%\usepackage{algorithm2e}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{xcolor}
\usepackage[colorinlistoftodos]{todonotes}


% \usepackage{hyperref}
%% natbib.sty is loaded by default. However, natbib options can be
%% provided with \biboptions{...} command. Following options are
%% valid:

\biboptions{sort,compress} 

\usepackage{xcolor}

% fixed line numbering
\newcommand*\patchAmsMathEnvironmentForLineno[1]{%
  \expandafter\let\csname old#1\expandafter\endcsname\csname #1\endcsname
  \expandafter\let\csname oldend#1\expandafter\endcsname\csname end#1\endcsname
  \renewenvironment{#1}%
     {\linenomath\csname old#1\endcsname}%
     {\csname oldend#1\endcsname\endlinenomath}}% 
\newcommand*\patchBothAmsMathEnvironmentsForLineno[1]{%
  \patchAmsMathEnvironmentForLineno{#1}%
  \patchAmsMathEnvironmentForLineno{#1*}}%
\AtBeginDocument{%
\patchBothAmsMathEnvironmentsForLineno{equation}%
\patchBothAmsMathEnvironmentsForLineno{align}%
\patchBothAmsMathEnvironmentsForLineno{flalign}%
\patchBothAmsMathEnvironmentsForLineno{alignat}%
\patchBothAmsMathEnvironmentsForLineno{gather}%
\patchBothAmsMathEnvironmentsForLineno{multline}%
}

\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{bbm}
\usepackage{lineno}
\usepackage{fullpage}
% for inline annotation
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{url}
% \usepackage[round]{natbib}
\usepackage{listings}
\usepackage[colorlinks=true]{hyperref}
\newtheorem{theorem}{Theorem}[]
\newtheorem{remark}{Remark}[]



\usepackage{color,soul}
\usepackage{enumitem}
\usepackage{mathtools}

% Collaboration tools
\definecolor{lightblue}{rgb}{.90,.95,1}
\definecolor{darkgreen}{rgb}{0,.5,0.5}


%indicates who is to lead the writing
%input is a list of names
\newcommand\assignment[1]{\todo[inline,color=red!10,size=\normalsize]{#1}}

%Indicates guides for what should be written
%input 2 is the guide text, #1 is the people leading the writing

\newcommand\guide[2]{\sethlcolor{lightblue}\hl{#2}\todo[color=lightblue,size=\tiny]{#1}}

%same as \guide but with no assignment
\newcommand\guidenoa[1]{\sethlcolor{lightblue}\hl{#1}}

\definecolor{lightgreen}{rgb}{.90,1,0.90}
\newcommand\bcon[1]{\todo[color=lightgreen,size=\tiny]{$\downarrow\downarrow\downarrow$ #1}}
\newcommand\econ[1]{\todo[color=lightgreen,size=\tiny]{$\uparrow\uparrow\uparrow$ #1}}

\newcommand\commofA[2]{\todo[color=red!50,size=\small,inline]{{\bf \color{blue} {#1}'s comments}:
    #2}}
\newcommand\commofB[2]{\todo[color=blue!50,size=\small,inline]{{\bf \color{blue} {#1}'s comments}: #2}}
\newcommand\commofC[2]{\todo[color=purple!50,size=\small,inline]{{\bf \color{blue} {#1}'s comments}:  #2}}

\newcommand{\bstau}{\boldsymbol{\tau}}
\newcommand{\bstaurans}{\tilde{\boldsymbol{\tau}}^{rans}}
\newcommand{\bs}[1]{\boldsymbol{#1}}
\newcommand{\missingref}{\textbf{[ref]}}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../rmt-main.tex"
%%% End: 


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../mfu-main"
%%% End: 



==> outline.tex <==
\textbf{Outline} \\
\begin{itemize}
\color{ForestGreen}
\item cardiovascualr disease is important 1 
\item CT,MRI provide information but no flow field. Image-based CFD gives functional information. image -based cfd expensive, not good for many query. 2-9 
\item ROM reduce cost, but no local details. previous work... 9-12
\item Alternative is interpolation-based surrogate model method.one formulation is to use dimension reduction tool to transfer highly non-linear CFD reuslts to low order latenet space. Then use a NN as a blackbox to map the input and the output. 13-16
\item Another formulation is to use hierarchy model such as Multi-fidelity surrogate models. The MF model is pioneered by ....  It leverage both ... from HF and ... from LF. 17-20
\item Current work on surrogate models are easy for parameterization, but 3d-geometry is hard to to parameterize. How to find a good way to parameterize the input shape and fully explore the input space? Plus, We developed SSM model to fully explore the input space.21-25
\end{itemize}

==> trash.tex <==


One crucial premise of geometry parameterization is building shape correspondence, where a point-to-point correspondence is found between two arbitrary aorta geometry shapes.  To obtain this correspondence, we used the nonparametric framework Deformetrica\cite{durrleman2014morphometry}. This framework is based on large deformation diffeomorphic metric mapping(LDDMM) algorithm\cite{beg2005computing}, which is capable of simultaneously computing the mean shape (template) of multiple shapes and subsequently the deformations from the mean shape to every other shape in the dataset. The algorithm is based on the idea of selecting the shortest length corresponding to geodesic flows. The mathematical form of the algorithm is provided in the cited literature above and we focus on its application in our experiments. Since the deformed shapes are almost identical to their original counterpart, we substitute the original geometries with those deformed shapes. Thus all samples are correlated.

In this study, we created an SSM model to generate synthetic shapes from corresponded shapes. The SSM uses PCA decomposition on shapes in the dataset and captures a few most significant eigenvectors. Each shape's projection on these eigenvectors is its encoded information. As used in \cite{liang2017machine}, we mathematically describe the process as following. Let $X=[x^1, x^2,\cdots, x^M]\in \mathbb{R}^{3N\times M}$ be the shape data set and each $x^m\in\mathbb{R}^{3N}$ for $m\in \{1, \cdots, M\}$ is a shape's mesh. Therefore, we can find $M$ eigenvectors and eigenvalues for these shapes, denote ad $\{V^1, \cdots, V^M\}$ and $\{\lambda_1, \cdots, \lambda_M\}$. With this setup, we can generate synthetic shapes by using $\Tilde{x}=\sum_{i=1}^K\alpha_i\lambda_i V^i$, where $\alpha_i$ are random numbers that follow some distribution and $K\leq M$ is the cap manually selected to meet our precision need. 

For any synthetic shape $\Tilde{x}\in\mathbb{R}^{3N}$, regardless of how it was generated, we can use $\alpha_1, \cdots, \alpha_K$, where $\alpha_i=\langle \Tilde{x},V^i \rangle/\lambda_i$ for $i\in {1,\cdots, K}$, as low dimensional embedding vector for the high dimensional surface mesh.

Subsequently, we use the simpleFoam solver to conduct a steady-state simulation on the prepared mesh via parallel processing. The field of interests (e.g. pressure, velocity, wall shear stress) are extracted from the simulation and given to the DNN-based surrogate model as ground truth. 

Since the optimization requires a massive parallelism of different trials, the Asynchronous Successive Halving Algorithm (ASHA) is used to aggressively terminate non-ideal trials in advance to save as much time as possible. More details of the ASHA can be found in \cite{LiASHA}. 

@article{LiASHA,
  title={ A system for massively parallel hyperparameter tuning},
  author={Li L, Jamieson K, Rostamizadeh A, Gonina E, Ben-Tzur J, Hardt M, Recht B, Talwalkar A.},
  journal={Proceedings of Machine Learning and Systems},
  volume={2},
  number={},
  pages={230-246},
  year={2020},
  publisher={}
}



Then MLP used Rectified Linear Unit (Relu) as the activation function and contains two hidden layers. Each field is connected to the shape inputs via individual MLP, including pressure, velocity and wall shear stress. Denote that the velocity vector field is separated into three scalar fields which are linked to the shape code using three different MLP. Whereas the wall shear stress values with N nodes are flattened into a column vector with the size of 3N, and then piped to the MLP. 

For optimization of the parameters in the MLP, we performed a distributed experiment to determine the value of the hyper-parameters. The tunable parameters include the dimensions of each hidden layer, the batch number and the learning rate of the ADAM optimizer. 100 experiments are conducted for each training mission, from which the best configuration of the hyper-parameter set will be picked out as the parameter settings for the final result. Such algorithm is realized by a open-source code package called RAY.  



SMM model is applied to achieve the parameterization of 3-D aorta geometry manifolds. Prior to the synthesis of artificial aorta shapes, correspondence are established among different curved surfaces. Figure 3 illustrates the process of building such correspondence between two arbitrary geometries: aorta $A_1$ serves as the source geometry and was sampled with a sufficient amount of points to guarantee the topological characteristics are fully captured. Then a function $\Phi(t)$ describing the diffeomorphism from source  is solved with $\Phi(t=0)$ and $\Phi(t=1)$ representing the surface vertices $P_1$ and $P_2$ respectively. Note that $P_2$ is obtained by minimizing the difference between itself and the target geometry $A_2$. During the diffeomorphism, intermediate shapes between the initial and final state of $\Phi(t)$ can be captured as synthetic geometry samples ready to be added into the aorta geometry dataset. 



In this work, the synthesizing method is applied on eight original geometries. The correspondence is found by the following process: one geometry is first selected as the template with 4000 vertices sampled on its surface, then a diffeomorphism function is solved from the template to each of the rest of the original geometries. A uniform sampling algorithm is used for the synthesis of new shapes: PCA transform is first used to convert the original geometries in to latent space. Boundaries of the first finite numbers of primary components are obtained. New sets of primary values are sampled from the regimes of the primary components via uniform distribution. The purpose of using uniform distribution is to fully explore the variation of the parameter space. Finally, applying inverse PCA transformation to the new value sets yields synthetic geometries. A total of 1000 samples are created in this work. Figure 4a illustrates the distribution of samples in the parameter space with the horizontal and vertical axis representing the first and second primary component values respectively. Both the original and the synthetic geometries are visualized in figure 4b.




bifidelity's advantage is more obvious, because it introduce more physical prior, but it requires more meshing and case set up. 
NN is comparable with Bifidelity models, 
Dont highlight deep learning, change it into machinge learin. 
parameterilization of input space. 

Idea: real simulation do karmen filter, find geom mean, then local region parameterize, and build NN, then use this surrogate to do MCMC, inferrring geometry uncertainty. 


Next paper, UQ inverse problem infering geometries is tricky. 


discussion
\subsection{SSM results}
Figure \ref{fig:sample_generate} demonstrates how synthetic geometries are generated from the original dataset in the case of 3 original geometries. The vertices of the triangle represent 3 original geometries. By randomly sampling values on primary components, 10 new synthetic shapes are created which are visualized by blue dots in the figure. By plotting all the samples on the first two primary components, one can observe that the distribution of the sample covers the interior of the triangle and the geometric shape of the new samples is shown at the bottom of the figure. From the shape, we can conclude that the synthetic geometries are like intermediate geometries that share similar geodesic characteristics from the original sample. For example, the point near real aorta 1 corresponding to the bottom left of the synthetic aorta also tends to have a large ascending aorta as well. 




Figure \ref{fig:sample_dist} shows the application of SSM in the case of 8 original geometries, where 600 new samples are randomly generated. The black, blue and red dots represent original samples, training samples and test samples respectively, which are plotted in a t-SNE plot that indicates the distance between samples distributed within the sample space. It appears that the samples fully occupied the space bounded by the original samples, which means that the training dataset ideally approximates the initial sample space. The proportions of the training dataset and test dataset are 80 percent and 20 percent. 



 As expected, the errors decrease as the proportion of the training set increases. For example, the pressure error climbs from $1.5\%$ to $4.5\%$ from $50\%$ training samples to $90\%$. 


C, where A cause B.
C, due to B which is caused by A.
C, where A -> B

A->B->C

eat too much -> fat -> affect social life -> no friends. 

Those who eat to much tend to get out of shape, which affect their social life and probably even isolate them from friends and relatives.
Note that each condition is repeated from 10 times with different initialization of the neural network and the averaged of those trials are reported.

\begin{center}
\begin{tabular}{ c c c c c c} 
 \hline
 Error(MSE) & Pressure & Velocity & Velocity Magnitude & WSS & WSS Magnitude \\
 \hline
 Test set & 1.336\% & 0.640\% & 0.438\% & 1.712\% & 1.248\% \\
 \hline
\end{tabular}
\end{center}


One process is accomplish in three steps: (1) (2) (3)
the process of ... is three-fold: 
the process consist of three steps:
the process is summarized as follow:
the process is formulated as follow: 
is delineate, 



The distribution of samples along PC1 (x) and PC2 (y) are shown in figure 4.



x->PC1; y->PC2


The relationship between the sample size and error is shown in figure 5. At 900 sample, both model have low error. when 
the samples size decreases, the error of model 1 (blue curve) rockets while that of model 2 stays on the same level/rises mildly. The poor performance of model 1 at small size results from its unrealistic assumptions. 




Consequently, the error is mild for smooth geometry like sample 23.  
For WSS contours, the situation is similar to the pressure contours. The low shear stress area is smaller in the predicted results compared to the ground truth. Other than that, the general pattern and the magnitude are in good agreement with each other.  

In terms of the velocity, the third row of figure 4 shows the velocity magnitude contour at the coronal cross-section, from which one can see a similar distribution of velocity between prediction and ground truth. At the stenosis of descending aorta for sample 4, the velocity of the prediction appears to attenuate the unsteadiness within this area. The nature of DNN is an interpolation between known samples, and such interpolation tends to smooth out large gradients for extreme samples like sample 4. 

From the 3D vector field plots, the magnitude and orientation of the velocity in the prediction are very close to the ground truth. However, one can identify small vortexes emerging near the area which the surrogate model did not accurately capture. One possible reason for this phenomenon is the limitation of the PCA since it directly applies dimension reduction on 3-D point clouds. It is possible that with the use of a more sophisticated shape encoder and field decoder that more accurately represents the curvature change of vessel wall, the error might be improved. 

